Chatperone: An LLM-Based Negotiable Scaffolding System for Mediating Adolescent Mobile Interactions

Adolescents' uncontrolled exposure to digital content can negatively impact their development. Traditional regulatory methods, such as time limits or app restrictions, often take a rigid approach, ignoring adolescents' decision-making abilities. Another issue is the lack of content and services tailored for adolescents. To address this, we propose Chatperone, a concept of a system that provides adaptive scaffolding to support adolescents. Chatperone fosters healthy mobile interactions through three key modules: Perception, Negotiation, and Moderation. This paper outlines these modules' functionalities and discusses considerations for real-world implementation.

==> hislab_commons/demos.tex <==
\section{Demo of common commands}
\begin{enumerate}
    \item \is{Example comment}
    \item \sj{Example comment}
    \item \je{Example comment}
    \item \jw{Example comment}
    \item \hj{Example comment}
    \item \cjw{Example comment}
    \item \jh{Example comment}
    \item \mg{Example comment}
    \item \sw{Example comment}
    \item \ks{Example comment}
    \item \kdh{Example comment}
    \item \dy{Example comment}
    \item \suwon{Example comment}
\end{enumerate}

This is \textbackslash userquote: \userquote{P1}{This is awesome!}

This is \textbackslash blueboxed: \blueboxed{Paint it blue!}

This is \textbackslash myquote:
\begin{myquote}{0.3in}
    \texttt{Our whole universe was in a hot, dense state
    Then nearly fourteen billion years ago expansion started, wait
    The earth began to cool, the autotrophs began to drool
    Neanderthals developed tools
    We built a wall (we built the pyramids)
    Math, science, history, unraveling the mysteries
    That all started with the big bang (bang)}
\end{myquote}

This is \textbackslash needfigure: Figure~\needfig{} depicts the architecture. 

This is \textbackslash needchart: Figure~\needchart{} plots the distribution.

This is \textbackslash needtable: Table~\needtable{} lists the accuracy measures.

This is \textbackslash needcite: Numerous reports testify I am handsome~\needcite{}.

This is \textbackslash unknown: Our peak accuracy is as high as \unknown{}\%.

==> hislab_commons/stats.tex <==
%TC:ignore
\debug{
\section{Debug Statistics}
Word Count - \quickwordcount{main} \\
Unknowns - \arabic{unknowncounter} \\
Comments - \arabic{commentcounter} \\
Need charts - \arabic{needchartcounter} \\
Need figures - \arabic{needfigcounter} \\
Need tables - \arabic{needtablecounter} \\
Need cites - \arabic{needcitecounter}
}
%TC:endignore

==> sections/02_related_work.tex <==
\section{Related Work}
\label{sec:related-work}


